Safe learning-based control via function-based uncertainty quantification

Uncertainty quantification is essential when deploying learning-based control methods in safety-critical systems. This is commonly realized by constructing uncertainty tubes that enclose the unknown function of interest, e.g., the reward and constraint functions or the underlying dynamics model, with high probability. However, existing approaches for uncertainty quantification typically rely on restrictive assumptions that encode smoothness properties of the unknown function, such as a known norm in a function space. Moreover, these methods usually struggle with discontinuities. In this paper, we model the unknown function as a random function from which independent and identically distributed realizations can be generated. We then construct uncertainty tubes via the scenario approach that hold with high probability. Our uncertainty tubes rely solely on sampled realizations and can therefore accommodate discontinuities represented by the sampling model. We integrate these uncertainty tubes into a safe Bayesian optimization algorithm with which we safely tune control parameters on a real Furuta pendulum.

==> Figures/intro.tex <==
% Preamble:
% \usepackage{tikz}
% \usetikzlibrary{arrows.meta,positioning}
% \usepackage{graphicx}

\begin{figure}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  box/.style={
    draw,
    rounded corners=2pt,
    thick,
    align=left,
    text width=0.85\linewidth,
    inner xsep=4mm,
    inner ysep=2mm
  },
  arrow/.style={-Latex, thick},
  node distance=6mm
]

\node[box] (I) {\textbf{I.} Function~$f:\domain\subseteq \mathbb R^n \mapsto \mathbb R$ maps control parameters to associated reward.};

\node[box, below=of I] (II) {\textbf{II.} The reward~$f$ is a random element of a probability space and we can sample~$f$ by conducting experiments subject to observation noise.};

\node[box, below=of II] (III) {\textbf{III.} 
\funsa: \textbf{F}unction-based \textbf{un}certainty quantification via the \textbf scenario \textbf approach: 
\[
f(a) \in [\ell(a),\, u(a)], \quad \text{w.h.p.}
\]};

\node[box, below=of III] (IV) {\textbf{IV.} We use \funsa\ for safe BO to optimize the performance of a Furuta pendulum.};

\draw[arrow] (I) -- (II);
\draw[arrow] (II) -- (III);
\draw[arrow] (III) -- (IV);

\end{tikzpicture}%
}
\caption{Logical structure from random-function modeling to safe Bayesian optimization.}
\label{fig:logic_flow}
\end{figure}


==> Figures/structure.tex <==
% Preamble

\begin{figure}[h!]
\centering
%\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
    transform shape,
    font=\normalsize,
    arrow/.style={->, line width=0.9pt},
    panel/.style={rectangle, fill=aaltoGray!60, inner sep=5mm},
    box/.style={rectangle, fill=white, minimum height=9mm, draw=black, align=center}
]

% ---------- Width parameters ----------
\def\distance{6}
\def\W{7} \def\BW{6} \def\SW{3}


% ================= TOP PANEL =====*============
\node[
    panel,
    minimum width=8cm,
    fill=aaltoGray!20,
    draw=black,
    inner sep=6pt
] (P1) {%
\begin{minipage}{7cm}
\centering
\textbf{Sec.~\ref{sec:modeling}: Probabilistic function modeling}

\vspace{2mm}

\begin{itemize}[left=0em]
\item  \small{Function representation via basis expansion with random coefficients (Asm.~\ref{asm:prob}, Sec.~\ref{sec:function-based-UQ})}
\item  \small{Generation of function scenarios by sampling coefficients from conditional distribution (Sec~\ref{sec:posterior}).}
\end{itemize}

\end{minipage}
};

% ===== Section I / II labels =====
\node[
    box,
    minimum width=4cm,
    above left=1mm and 0mm of P1.north
] (S1)
{Sec.~\ref{sec:introduction}: Introduction};

\node[
    box,
    minimum width=4cm,
    above right=1 mm and 0mm of P1.north
] (S2)
{Sec.~\ref{sec:problem_setting}: Problem setting};


% ================= MIDDLE PANEL =====*===========
\node[
    panel,
    minimum width=8cm,
    below=\distance mm of P1,
    fill=aaltoGray!60,
    inner sep=6pt,
    draw=black
] (P2) {%
\begin{minipage}{7cm}
\centering
\textbf{Sec.~\ref{sec:tube}: Constructing uncertainty tubes}

\vspace{2mm}

\begin{itemize}[left=0em]
\item \small{Based on theory of classic scenario approach~\cite{campi2018introduction} (Thm.\ref{th:classic_scenario}) and wait-and-judge framework~\cite{campi2018wait} (Thm.\ref{th:uncertainty_tubes})}
\end{itemize}

\end{minipage}
};


    \node[box, minimum width=8cm, below=\distance mm of P2, fill=aaltoGray!20] (P3)
      {Sec.~\ref{sec:BO}: Safe Bayesian optimization};

    \node[box, minimum width=8cm, below=\distance mm of P3, fill=aaltoGray!20] (P4)
      {Sec.~\ref{sec:exp}: Safe control parameter tuning experiments};

    \node[box, minimum width=8cm, below=1 mm of P4] (X)
      {Sec.~\ref{sec:conclusion}: Concluding remarks and future work};


% ----- Arrows -----
\draw[arrow] (P1.south) -- node[right]{Function-based UQ} (P2.north);
\draw[arrow] (P2.south) -- node[right]{Uncertainty tubes} (P3.north);
\draw[arrow] (P3.south) -- node[right]{Safe BO algorithm} (P4.north);

\end{tikzpicture}%
%}
\caption{High-level illustration of this article.
}
\label{fig:intro}
\end{figure}


==> Sections/problem_setting.tex <==
%\section{PROBLEM SETTING}
We consider functions that map from a discrete domain to the real numbers,
\[
f:\domain\subseteq\mathbb R^n \to \mathbb R,
\qquad |\domain|<\infty .
\]
Let $(\Omega,\mathcal B(\Omega),\mu)$ denote the underlying probability space,
where $\Omega$ is the sample space, $\mathcal B(\Omega)$ is its Borel
$\sigma$-algebra, and $\mu$ is the probability measure.
We interpret functions as random elements taking values in the measurable
function space
\[
\mathcal X := \{f:\domain\to\mathbb R\},
\]
which we identify with $\mathbb R^{|\domain|}$ by associating each function
with its vector of values on the grid points. We equip
$(\mathcal X,\mathcal B(\mathcal X))$ with the Borel $\sigma$-algebra
$\mathcal B(\mathcal X)=\mathcal B(\mathbb R^{|\domain|})$.

A \emph{random function} is a measurable mapping
\[
F : (\Omega,\mathcal B(\Omega)) \to (\mathcal X,\mathcal B(\mathcal X)).
\]
For each outcome $\omega\in\Omega$, the value $F(\omega)\in\mathcal X$ is a full
discrete function on~$\domain$; we denote such realizations by $f$. Since
$\mathcal X \cong \mathbb R^{|\domain|}$, this corresponds to
\[
F(\omega)
=
\big(F(\omega)(x_1),\dots,F(\omega)(x_{|\domain|})\big)
\in\mathbb R^{|\domain|}.
\]

The probability law of the random function $F$ on the function space
$\mathcal X$ is given by the pushforward measure
\[
\mu_F := \mu \circ F^{-1}.
\]

Scenario functions are modeled as i.i.d.\ copies of the same measurable map,
that is,
\[
F,\,G_1,\dots,G_N \text{ are i.i.d.\ random functions with common law } \mu_F .
\]

In our setting, the choice of the law $\mu_F$ on the function space
$(\mathcal X,\mathcal B(\mathcal X))$ is left generic, and different
stochastic models for random functions can be accommodated. Typical
examples include the following classes:
\begin{itemize}
    \item Samples from a Gaussian process
    \item Samples from a Markov process (Poission, Lévy)
    \item Solution to a stochastic partial differential equation
\end{itemize}

All functions are then of the form:
\begin{align}
    f(a)=\sum_{i=1}^N\alpha_i \varphi(a),
\end{align}
where~$\varphi(\cdot)$ is fixed and~$\alpha_i$ is random.
Knowing the probability space allows sampling from it and deriving uncertainty tubes.
Since we have a discrete domain, the Kosambi--Karhunen-Loève (KKL) expansion is exact and we can draw random functions from that probability space, \eg by just drawing Gaussians $\alpha_i$ with RKHS basis functions \refneeded.

This is parametric. 
Non-parametric is Gaussian process~\cite{williams2006gaussian}, or e.g., Student's-$t$~\cite{shah2014student}.
Advantage: the approximating function can be anything, we need basis functions instead of the kernel; which is just a little bit different.
We could also have Gaussian process or Student's-$t$ process through KKL expansion, but we need samples from the probability space; and we can only create finite sums. 
What about infinite sums?


\begin{assumption}[Epistemic uncertainty]\label{asm:prob}
    The ground truth function~$f:\mathbb A\mapsto\mathbb R^n$ and the random functions~$\rho_{j,t}$ are independent and identically distributed (i.i.d.) samples from the same probability space.
\end{assumption}


\begin{definition}[Random functions]\label{def:random_function}
    We mean by a random function to be of the form
        $f(a)=\sum_{i=1}^{\lvert \domain \rvert} \alpha_i \varphi_i(a)$. 
        The basis functions are fixed and known and can be anything.
        The coefficients~$\alpha_i$ are random and are sampled from a probability space conditioned on the observed sample pairs $(a_{1:t}, y_{1:t})$, where $y_{t}=f(a_t)+\epsilon_t$ with~$\epsilon_t$ according to Assumption~\ref{asm:noise}.
        Since~$y_{1:t}$ is endowed by measurement noise, we do not want to interpolate~$(a_{1:t}, y_{1:t})$ directly but instead interpolate through~$y_t + \tilde\epsilon_t$, where~$\tilde\epsilon_t\in (\Omega_\epsilon, \mathcal F_\epsilon, \mathbb P_\epsilon)$.
        In the Gaussian process setting, this posterior is fully defined~\cite{williams2006gaussian}, but otherwise not.
        We take a uniform view on this probability space that works across observation noise models.
    We sample the coefficients according to
    \begin{align*}
        \alpha \sim \mathbb P_\alpha (\cdot \vert \rho_j(a_t)=y_t+\tilde\epsilon_t)
    \end{align*}
We are projecting the probability space down to the interpolation subset in the following way:
\end{definition}





Assumption~\ref{asm:prob} shits the uncertainty to the function, unified, allows to give marginal Bayesian type guarantees.
We will make this assumption more precise later.

\begin{assumption}[Aleatoric uncertainty]\label{asm:noise}
    The observation noise~$\epsilon_t$ is a sample from a probability space $(\Omega_\epsilon, \mathcal F_\epsilon, \mathbb P\epsilon)$, from which we can sample.
\end{assumption}
Assumption~\ref{asm:noise} is equivalent to \cite[Assumption~1]{tokmak2026safe}, where noise scenarios~$\tilde\epsilon_t$ are sampled to compute a high probability bound on the observation noise~$\epsilon_t$.
In this setting, we do not require a bound on the observation noise since the previous work was based on bounding an RKHS term and a noise term.
Now we just create trajectories and get our bounds from there.



\textbf{Other validation methods:}
\begin{itemize}
    \item Other scenario-based approaches: See Simone's email, maybe we will use constraint relaxation in a non-convex setting, then there is constraint discarding and the classic convex setting. Pick to learn? \cite{garatti2025non}, \cite{campi2018introduction}, \cite{paccagnan2025pick}
    \item Definitely conformal prediction: \cite{lindemann2024formal}, \cite{vovk2005algorithmic}; also see connection: \cite{o2025bridging}
    \item \url{https://arxiv.org/pdf/1509.07526}, \url{https://mogp-emulator.readthedocs.io/en/latest/methods/disc/DiscKarhunenLoeveExpansion.html},
    \url{https://www.cs.cmu.edu/~andrewgw/tprocess.pdf}
\end{itemize}




\textbf{Incorporating aleatoric uncertainty}
\begin{itemize}
    \item Does not really matter what we choose as long as we treat epistemic and aleatoric uncertainty to be independent, we can construct a product probability space to formulate joint probabilities
    \item  We can take the scenario approach formulation from \cite{tokmak2025safe} because it fits into the whole story
    \item In GPs, we can condition on the data and it gives an analytical formula
\end{itemize}


==> Sections/safe_BO.tex <==


\safeopt\ but we are a bit different and also better, definitely better than~\cite{tokmak2025safe}
Safe BO control parameter tuning with Furuta pendulum~\cite{furuta1992swing}.
We compare to classic \safeopt~\cite{sui2015safe}, \pacsbo~\cite{tokmak2025safe} and show that we have less assumptions and tighter bounds than \cite{tokmak2025safe} and do not require RKHS norm but we are in a different setting.


\begin{align*}
    p_t(x)=\ell_t(x)+(u_t(x)-\ell_t(x))\sigma_t(x),
\end{align*}
where~$\sigma_t(x)\in[0,1]$ by construction and learned by a NN, and since by construction we have $p_t(x)\in[\ell_t(x),u_t(x)]$, we have ``safety with high probability.''

==> Sections/scalar.tex <==
%\section{Warm-up: Scalar function-based UQ}



In this section, we derive uncertainty bounds for \emph{scalar} functionals of random functions like their Lipschitz constant. 
A bound on the Lipschitz constant or the functional norm---like the RKHS norm---is of independent interest in learning and control; see~\cite{xue2022chordal, wood1996estimation} for Lipschitz constant and~\cite{tokmak2024pacsbo, tokmak2025safe, tokmak2025automatic} for RKHS norm estimations.
These bounds quantify the behavior of the unknown function with high probability, which can then yield safety guarantees in exploration~\cite{sui2015safe, berkenkamp2023bayesian, turchetta2019safe}.
Unlike~\eqref{eq:tube}, where we aim to control~$h_i$ from escaping the uncertainty tube over the domain, restricting ourselves to only scalar characteristics of~$h_i$ simplifies the task.
Nonetheless, the reader is invited to bear with us; this reduced setting already exhibits the key mathematical structure available under Assumptions~\ref{asm:noise} and~\ref{asm:prob} and allows us to introduce the main analytical tool---the scenario approach~\cite{campi2018wait}---which we will subsequently use to satisfy~\eqref{eq:tube} in Section~\ref{sec:tube}.


%Next, we will present the main result of this section.
Let us denote by~$\mathcal S$ a scalar measurable functional  $\mathcal S: (\R^{\lvert\domain\rvert}, \mathcal B(\R^{\lvert\domain\rvert})) \to (\R, \mathcal B(\R))$ that we aim to over-estimate\footnote{%
Equivalently under. These methods offer one-sided bounds, we could combine to interval probably and use the negation of it for lower bounds, but here now just upper. 
} and by~$\lceil \xi \rceil$ as rounding~$\xi\in\R$ up to the next integer.
%, which can, \eg map a function to its Lipschitz constant, RKHS norm, numerical integral, supremum, or infimum, whose functionals we denote by~$\mathcal S_\mathrm{L}, \mathcal S_\mathrm{R}, \mathcal S_\mathrm{int}, \mathcal S_\mathrm{sup}$, and $\mathcal S_\mathrm{inf}$, respectively.
The following theorem proves that we can construct an interval that contains~$S(h_i)$ with high probability, solely by computing the functional~$S(\rho_{i,t}^\jj)$ of the random functions~$\rho_{i,t}^\jj$.


\begin{theorem}[General scalar functionals]\label{th:general_scalar}
    Let Assumptions~\ref{asm:noise} and~\ref{asm:prob} hold and choose any probability level~$\nu\in(0,1)$ and any confidence level~$\kappa\in (0,1)$.
    For any~$t\geq 1$, generate~$m_t\in\mathbb N$ i.i.d.\ scenarios~$\rho_t^\jj$, with~$m_t$ satisfying
    \begin{align*}
    \min_{m_t\in\mathbb N} m_t \quad 
    \text{s.t.} \quad    \sum_{i=0}^{m_t-p_t} {m_t\choose i}\nu^i (1-\nu)^{m_t-i}
    \leq \frac{6\kappa}{\pi^2t^2},
    \end{align*}
    where~$p_t = \lceil (1-\nu)(m_t-1)\rceil$.
Then,
    \begin{align}\label{eq:scalar_bound}
        \mathbb {\tilde P}[
        \forall t\geq 1: 
        \mathbb P[
        \mathcal S_i(f) \leq \mathcal S_i(\rho_t^{(p_t)})
        ]\geq 1-\nu
        ]\geq 1-\kappa.
    \end{align}
\end{theorem}

\begin{proof}
    The proof is divided into four parts.
    In Part~I, we show that a measurable and deterministic mapping of a random variable yields a random variable from an induced probability space and that this mapping preserves independence.
    In Part~II, we bound the obtained random variables via the scenario approach by using the sampled random functions.
    In Part~III, we lift these bounds to holds simultaneously for all iterations~$t\geq 1$ using a classic union bound.

    \textbf{Part~I:}
        First, we prove that the scalar functionals of~$f$ are random variables (the same applies to~$\rho_t^\jj$ mutatis mutandis) before proving that~$S(f)$ and~$S(\rho_t^\jj)$ are i.i.d.
    All aforementioned functionals~$S(f)$ are deterministic and continuous mappings and continuous mappings are measurable~\cite[Exercise~1.3.4]{durrett2019probability}, \cite[Section~7]{tokmak2024pacsbo}.
    Therefore,~$S(f)$ is a deterministic and measurable mapping of a random variable~$f$, and hence~$S(f)$ is a random variable itself, see \eg \cite[Theorem~1.3.5]{durrett2019probability}  for the general result and~\cite[Theorem~1.3.7]{durrett2019probability} for the result on the infimum and the supremum.
%
Independence: Measurable and deterministic function does not influence the $\sigma$-algebras and therefore independence and distribution stay the same. So the distribution becomes an induced distribution. 
\AT{To make it more clear use the concatenation of~\cite[Theoren~1.3.4]{durrett2019probability}}.    
\end{proof}

Theorem~\ref{th:general_scalar} allows us to bound any measurable scalar quantity of the unknown function~$f$. 
The following corollary lists a handful of interesting scalar functionals that we can bound as a direct result of Theorem~\ref{th:general_scalar}.

\begin{corollary}[Specific scalar functionals]\label{co:specific_scalar}
    Under the same hypotheses as those of Theorem~\ref{th:general_scalar}, consider now the following scalar quantities with corresponding functionals:
    \begin{itemize}
    \item Lipschitz constant $S_\mathrm{L}(f)\coloneqq \max\limits_{a,a^\prime\in\domain, a\neq a^\prime}\frac{\lvert f(a)-f(a^\prime)}{\|a-a^\prime\|}$;
    \item RKHS norm \AT{Should be included since cf. \cite{tokmak2025safe}};
    \item Numerical integral $S_{\mathrm{int}}\coloneqq \sum_{i=1}^{\lvert\domain\rvert-1}(a_{i+1} - a_{i})f(a_i)$;
    \item Supremum $S_{\sup}(f)\coloneqq \sup_{a\in\domain} f(a)$;
    \item Infimum $S_{\inf} (f)\coloneqq \inf_{a\in\domain} f(a)$
\end{itemize}
Then, upper and lower bounds like~\eqref{eq:scalar_bound} are achievable.
\end{corollary}
\begin{proof}
    Just proof that they are i.i.d.\ random variables.
\end{proof}


Inside the first long proof:
\begin{itemize}
    \item With this, introduce the scenario program very naturally 
    \item We know that they are i.i.d.\ and then the scenario approach can give us generalization guarantees
    \item Write down briefly the scenario approach or the violation probability and the guarantees that the scenario approach gives
    \item Write that it is based on Helly's theorem~\cite{danzer1963helly}.
    \item Then say it is equivakent to order statistics, \eg conformal prediction~\cite{o2025bridging}, but necessary for us to reseive the full bounds we want
\end{itemize}








In this setting, conformal prediction and sampling-and-discarding scenario approach \cite{romao2022exact}, see \cite{o2025bridging}.
Here the key will be to show the potential application areas of function-based uncertainty quantification, but to also show that the scenario approach does not really yield anything better or worse than order statistics.


\begin{remark}[Theorem~\ref{th:general_scalar} and order statistics]
     If the object we want to bound truly reduces to a scalar quantity, the techniques that the scenario approach offers is even too much for the bounds.
    We can obtain completely equivalent results via order statistics, specifically via calibration-conditional conformal prediction.
    Conformal prediction has recently gained huge interest in the control community~\cite{lindemann2024formal}, and see~\cite{vovk2013conditional} for calibration-conditional conformal prediction and~\cite{o2025bridging} for the equivalence of this specific case.
    However, vanilla conformal prediction is not enough to reach the bounds we want in Section~\ref{sec:tube}.
\end{remark}

==> Sections/uncertainty_tubes.tex <==
\section{Probabilistic uncertainty tubes}
More interesting when we go towards confidence tubes to contain a function with high probability again.
We will apply this to safe Bayesian optimization (BO) and to something else.

Only GP setting: \cite[Lemma~5.1]{srinivas2012information}: Super bad credible intervals since they scale with the cardinality of the domain. But they give regret bounds on this, which we do not offer.


Distribution free prediction bands: \cite{lei2012distribution}, also cited in \cite{vovk2013conditional}


Conformal prediction with computable prediction bands: \cite{razafindrakoto2026approximate}


\subsection{Classic scenario theory}

\subsection{Parametrized scenario theory}


\subsection{Compression theory}
\begin{itemize}
    \item Is non-degeneracy a problem with interpolation? Might be? But not if we see the constraint as a vector and then they can be the same at some point as long as it is not a vector. And anyways, we will have noise of some sort.
    \item If non-degeneracy is a problem, we can use the non-convex scenario approach: \cite{garatti2025non}
    \item Can we discard constraints in the non-convex approach? (wait and judge principal, but with discarding?)
\end{itemize}


